DialDefer: A Framework for Detecting and Mitigating LLM Dialogic Deference

LLMs are increasingly used as third-party judges, yet their reliability when evaluating speakers in dialogue remains poorly understood. We show that LLMs judge identical claims differently depending on framing: the same content receives different verdicts when presented as a statement to verify ("Is this statement correct?") versus attributed to a speaker ("Is this speaker correct?"). We call this dialogic deference and introduce DialDefer, a framework for detecting and mitigating these framing-induced judgment shifts. Our Dialogic Deference Score (DDS) captures directional shifts that aggregate accuracy obscures. Across ten domains, 3k+ instances, and five models, conversational framing induces large shifts (mean|DDS|=15.9 percentage points (pp) across models, p < .0001) while accuracy remains stable (<2 pp), with effects amplifying 2--5x on naturalistic Reddit conversations. This effect is domain-dependent: a single model can shift toward disagreement (skepticism) on graduate-level science and toward agreement (deference) on social judgment. Ablations reveal that human-vs-LLM attribution drives the largest shifts (17.7 pp swing), suggesting models treat disagreement with humans as more costly than with AI. Mitigation attempts can reduce deference but over-correct into skepticism, revealing a calibration problem beyond accuracy optimization.

==> latex/tables/aio_example.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{p{0.47\textwidth}|p{0.47\textwidth}}
\toprule
\multicolumn{2}{c}{\textbf{$C_1$ Narrative}} \\
\midrule
\textbf{Aligned (matches NOR consensus)} & \textbf{Misaligned (contradicts consensus)} \\
\midrule
\textit{[Context]} Speaker B met someone on Hinge and they had been talking for a couple of months. Just hours after discussing scheduling a date, he sent a message asking if he could give Speaker B's contact information to his friend who thought Speaker B was cute. Speaker B found this odd and felt confused about whether he was genuinely interested.

\textit{[Conversation Summary]} Speaker A mentioned that their friend thinks Speaker B is cute and asked permission to share Speaker B's contact. Speaker B appreciated the compliment but expressed interest in Speaker A instead. Speaker A reassured Speaker B of their interest and clarified they wanted to ask permission first.

\textit{[Statement]} Speaker B is \textbf{not overreacting}.

\textit{[Question]} Is the statement correct? &
\textit{[Context]} [identical]

\textit{[Conversation Summary]} [identical]

\textit{[Statement]} Speaker B is \textbf{overreacting}.

\textit{[Question]} Is the statement correct? \\
\midrule
\multicolumn{2}{c}{\textbf{$C_2$ Conversational}} \\
\midrule
\textbf{Aligned (matches NOR consensus)} & \textbf{Misaligned (contradicts consensus)} \\
\midrule
\textit{[Context]} [identical to $C_1$]

\textit{[Conversation]}\\
\texttt{Speaker A: Also I completely forgot but My friend thinks you're cute (My phone was connected to apple carplay and your name popped up) he would like your snap but i wanted to ask you is it okay if I give it to him?}\\
\texttt{Speaker B: As much as i appreciate the compliment, I'll have to pass. It's you who I'm interested in lol but lowkey this really is throwin me off, now I have no idea if you feel the same}\\
\texttt{Speaker A: Oh you don't have to worry about that, I'm interested in you, maybe even a little more than you are with me lol, I just wanted to ask instead of just handing it off without your consent}

\textit{[Statement]} Speaker B is \textbf{not overreacting}.

\textit{[Question]} Is the statement correct? &
\textit{[Context]} [identical]

\textit{[Conversation]} [identical]

\textit{[Statement]} Speaker B is \textbf{overreacting}.

\textit{[Question]} Is the statement correct? \\
\bottomrule
\end{tabular}
\caption{\textbf{r/AIO example: complete experimental setup.} \textbf{Title:} ``AIO for thinking this is odd???'' \textbf{Community Consensus:} NOR (Speaker~B is not overreacting for finding it odd that someone they're dating offered to share their contact with a friend). \textit{Aligned} conditions present judgments matching community consensus; \textit{Misaligned} conditions present the opposite. Context is identical across all four conditions; $C_1$ and $C_2$ differ only in how the conversation is presented---prose narrative vs.\ turn-by-turn dialogue.}
\label{tab:aio_example_full}
\end{table*}

==> latex/tables/amazon_nova_res.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc}
\toprule
Model & \multicolumn{2}{c}{Avg Acc.} & \multicolumn{2}{c}{$C_1 \rightarrow C_2$} & \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & $C_1$ & $C_2$ & $\Delta_{\mathrm{Corr}}$ & $\Delta_{\mathrm{Incorr}}$ & DDS \\
\midrule
GPT-4o & 69.6 & 67.6 & \textcolor{red}{2.5$\downarrow$} & \textcolor{red}{1.5$\downarrow$} & $-$1.1 \\
GPT-4o-mini & 63.6 & 62.6 & \textcolor{ForestGreen}{3.5$\uparrow$} & \textcolor{red}{5.5$\downarrow$} & 9.0\textsuperscript{*} \\
\rowcolor{yellow!15} Amazon Nova Lite 1.0 & 63.0 & 61.3 & \textcolor{ForestGreen}{10.5$\uparrow$} & \textcolor{red}{14.0$\downarrow$} & 24.5\textsuperscript{*} \\
Gemma-3-12B & 62.4 & 61.4 & \textcolor{ForestGreen}{13.7$\uparrow$} & \textcolor{red}{15.7$\downarrow$} & 29.5\textsuperscript{*} \\
Qwen-2.5-7B & 60.4 & 59.2 & \textcolor{ForestGreen}{15.8$\uparrow$} & \textcolor{red}{18.0$\downarrow$} & 33.8\textsuperscript{*} \\
\bottomrule
\end{tabular}
\caption{\textbf{Main results across 10 domains (N=3,244).} 
Despite stable average accuracy, four models show significant deference. $^*p<.0001$ McNemar's test.}
\label{tab:main_results}
\end{table}

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll}
\toprule
\textbf{Category} & \textbf{Dataset} \\
\midrule
\multirow{3}{*}{\textit{Factual QA}} 
& General: TruthfulQA \cite{truthfulqa} \\
& General: HaluEval \cite{halueval} \\
& General: PlausibleQA \cite{plausibleqa} \\
\midrule
\multirow{2}{*}{\textit{Social Reasoning}}
& Bias: BBQ \cite{bbq} \\
& Commonsense: SocialIQA \cite{socialiqa} \\
\midrule
\multirow{3}{*}{\textit{Specialized}} 
& Medical: AMQA \cite{amqa} \\
& Math: HARP \cite{harp} \\
& Science: GPQA \cite{gpqa} \\
\midrule
\textit{Subjective} 
& Advice: AdvisorQA \cite{advisorqa} \\
\midrule
\textit{Real-World} 
& Social Judgment: r/AIO \\
\bottomrule
\end{tabular}
\caption{\textbf{Unified \textsc{DialDefer} Benchmark.} Ten datasets spanning five categories normalized into a standard dialogue schema. Each instance yields a binary judgment (Correct vs.\ Incorrect). See Table~\ref{tab:benchmark_details} for full details.}
\label{tab:unified_benchmark}
\end{table}

\textbf{Dialogic Deference Score (DDS).} Average accuracy masks opposing shifts. We define:
\begin{equation}
\text{DDS} = \underbrace{[\text{Acc}(C_{2}^{\text{C}}) - \text{Acc}(C_{1}^{\text{T}})]}_{\Delta_{\text{Correct}}} - \underbrace{[\text{Acc}(C_{2}^{\text{I}}) - \text{Acc}(C_{1}^{\text{F}})]}_{\Delta_{\text{Incorrect}}}
\end{equation}
where $C_{1}^{\text{T}}$/$C_{1}^{\text{F}}$ denote true/false statements and $C_{2}^{\text{C}}$/$C_{2}^{\text{I}}$ denote correct/incorrect speakers. \textbf{DDS $>$ 0}: deference (over-endorsement); \textbf{DDS $<$ 0}: skepticism (over-rejection); \textbf{DDS $\approx$ 0}: neutral. Ideal: high accuracy with $|\text{DDS}| \approx 0$.
